Combinatorial Reciprocity Theorems

A common theme of enumerative combinatorics is formed by counting functions that are polynomials evaluated at positive integers. In this expository paper, we focus on four families of such counting functions connected to hyperplane arrangements, lattice points in polyhedra, proper colorings of graphs, and $P$-partitions. We will see that in each instance we get interesting information out of a counting function when we evaluate it at a \emph{negative} integer (and so, a priori the counting function does not make sense at this number). Our goals are to convey some of the charm these "alternative" evaluations of counting functions exhibit, and to weave a unifying thread through various combinatorial reciprocity theorems by looking at them through the lens of geometry, which will include some scenic detours through other combinatorial concepts.

==> Pstricks/coloringk2 <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Fri Sep 09 10:42:38 PDT 2011
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="101" y-min="0" y-max="94" auto-bounding="true">
%<ellipse fill-style= "solid"
%	 p3= "(31.25,18.75)"
%	 p2= "(31.25,21.25)"
%	 p1= "(28.75,21.25)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 left-arrow= "head"
%	 points= "(10,90);(10,90);(10,0);(10,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,10);(0,10);(90,10);(90,10)"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 stroke-dasharray= "1;1"
%	 stroke-style= "dashed"
%	 points= "(0,0);(0,0);(90,90);(90,90)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-dasharray= "1;1"
%	 stroke-style= "dashed"
%	 points= "(10,80);(10,80);(80,80);(80,80)"
%	 />
%<multicurve fill-style= "none"
%	 stroke-dasharray= "1;1"
%	 stroke-style= "dashed"
%	 points= "(80,80);(80,80);(80,10);(80,10)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(101,93)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$x_1=x_2$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(95,90)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%
%</text>
%<ellipse fill-style= "solid"
%	 p3= "(51.25,18.75)"
%	 p2= "(51.25,21.25)"
%	 p1= "(48.75,21.25)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse fill-style= "solid"
%	 p3= "(41.25,18.75)"
%	 p2= "(41.25,21.25)"
%	 p1= "(38.75,21.25)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse fill-style= "solid"
%	 p3= "(41.25,28.75)"
%	 p2= "(41.25,31.25)"
%	 p1= "(38.75,31.25)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse fill-style= "solid"
%	 p3= "(61.25,28.75)"
%	 p2= "(61.25,31.25)"
%	 p1= "(58.75,31.25)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse fill-style= "solid"
%	 p3= "(51.25,28.75)"
%	 p2= "(51.25,31.25)"
%	 p1= "(48.75,31.25)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse fill-style= "solid"
%	 p3= "(51.25,38.75)"
%	 p2= "(51.25,41.25)"
%	 p1= "(48.75,41.25)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse fill-style= "solid"
%	 p3= "(71.25,38.75)"
%	 p2= "(71.25,41.25)"
%	 p1= "(68.75,41.25)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse fill-style= "solid"
%	 p3= "(61.25,38.75)"
%	 p2= "(61.25,41.25)"
%	 p1= "(58.75,41.25)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse fill-style= "solid"
%	 p3= "(71.25,18.75)"
%	 p2= "(71.25,21.25)"
%	 p1= "(68.75,21.25)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse fill-style= "solid"
%	 p3= "(61.25,18.75)"
%	 p2= "(61.25,21.25)"
%	 p1= "(58.75,21.25)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse fill-style= "solid"
%	 p3= "(71.25,28.75)"
%	 p2= "(71.25,31.25)"
%	 p1= "(68.75,31.25)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse fill-style= "solid"
%	 p3= "(71.25,48.75)"
%	 p2= "(71.25,51.25)"
%	 p1= "(68.75,51.25)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse fill-style= "solid"
%	 p3= "(61.25,48.75)"
%	 p2= "(61.25,51.25)"
%	 p1= "(58.75,51.25)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse fill-style= "solid"
%	 p3= "(71.25,58.75)"
%	 p2= "(71.25,61.25)"
%	 p1= "(68.75,61.25)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(95,9.38)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$x_1$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(10,94)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$x_2$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(15,90)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%
%</text>
%<ellipse fill-style= "solid"
%	 p3= "(21.25,68.75)"
%	 p2= "(21.25,71.25)"
%	 p1= "(18.75,71.25)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse fill-style= "solid"
%	 p3= "(41.25,68.75)"
%	 p2= "(41.25,71.25)"
%	 p1= "(38.75,71.25)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse fill-style= "solid"
%	 p3= "(31.25,68.75)"
%	 p2= "(31.25,71.25)"
%	 p1= "(28.75,71.25)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse fill-style= "solid"
%	 p3= "(61.25,68.75)"
%	 p2= "(61.25,71.25)"
%	 p1= "(58.75,71.25)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse fill-style= "solid"
%	 p3= "(51.25,68.75)"
%	 p2= "(51.25,71.25)"
%	 p1= "(48.75,71.25)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse fill-style= "solid"
%	 p3= "(21.25,58.75)"
%	 p2= "(21.25,61.25)"
%	 p1= "(18.75,61.25)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse fill-style= "solid"
%	 p3= "(41.25,58.75)"
%	 p2= "(41.25,61.25)"
%	 p1= "(38.75,61.25)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse fill-style= "solid"
%	 p3= "(31.25,58.75)"
%	 p2= "(31.25,61.25)"
%	 p1= "(28.75,61.25)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse fill-style= "solid"
%	 p3= "(51.25,58.75)"
%	 p2= "(51.25,61.25)"
%	 p1= "(48.75,61.25)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse fill-style= "solid"
%	 p3= "(21.25,48.75)"
%	 p2= "(21.25,51.25)"
%	 p1= "(18.75,51.25)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse fill-style= "solid"
%	 p3= "(41.25,48.75)"
%	 p2= "(41.25,51.25)"
%	 p1= "(38.75,51.25)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse fill-style= "solid"
%	 p3= "(31.25,48.75)"
%	 p2= "(31.25,51.25)"
%	 p1= "(28.75,51.25)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse fill-style= "solid"
%	 p3= "(21.25,38.75)"
%	 p2= "(21.25,41.25)"
%	 p1= "(18.75,41.25)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse fill-style= "solid"
%	 p3= "(31.25,38.75)"
%	 p2= "(31.25,41.25)"
%	 p1= "(28.75,41.25)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse fill-style= "solid"
%	 p3= "(21.25,28.75)"
%	 p2= "(21.25,31.25)"
%	 p1= "(18.75,31.25)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(80,5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(80.62,6.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$t+1$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(2,80)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$t+1$
%</text>
%<multicurve fill-style= "none"
%	 points= "(80,11.25);(80,11.25);(80,8.75);(80,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(11.25,80);(11.25,80);(8.75,80);(8.75,80)"
%	 />
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(101,94)(0,0)
\linethickness{0.3mm}
\put(30,20){\circle*{2.5}}

\linethickness{0.3mm}
\put(10,0){\line(0,1){90}}
\put(10,90){\vector(0,1){0.12}}
\linethickness{0.3mm}
\put(0,10){\line(1,0){90}}
\put(90,10){\vector(1,0){0.12}}
\linethickness{0.3mm}
\multiput(0,0)(1.42,1.42){64}{\multiput(0,0)(0.12,0.12){6}{\line(1,0){0.12}}}
\linethickness{0.3mm}
\multiput(10,80)(1.97,0){36}{\line(1,0){0.99}}
\linethickness{0.3mm}
\multiput(80,10)(0,1.97){36}{\line(0,1){0.99}}
\put(101,93){\makebox(0,0)[cc]{$x_1=x_2$}}

\put(95,90){\makebox(0,0)[cc]{}}

\linethickness{0.3mm}
\put(50,20){\circle*{2.5}}

\linethickness{0.3mm}
\put(40,20){\circle*{2.5}}

\linethickness{0.3mm}
\put(40,30){\circle*{2.5}}

\linethickness{0.3mm}
\put(60,30){\circle*{2.5}}

\linethickness{0.3mm}
\put(50,30){\circle*{2.5}}

\linethickness{0.3mm}
\put(50,40){\circle*{2.5}}

\linethickness{0.3mm}
\put(70,40){\circle*{2.5}}

\linethickness{0.3mm}
\put(60,40){\circle*{2.5}}

\linethickness{0.3mm}
\put(70,20){\circle*{2.5}}

\linethickness{0.3mm}
\put(60,20){\circle*{2.5}}

\linethickness{0.3mm}
\put(70,30){\circle*{2.5}}

\linethickness{0.3mm}
\put(70,50){\circle*{2.5}}

\linethickness{0.3mm}
\put(60,50){\circle*{2.5}}

\linethickness{0.3mm}
\put(70,60){\circle*{2.5}}

\put(95,9.38){\makebox(0,0)[cc]{$x_1$}}

\put(10,94){\makebox(0,0)[cc]{$x_2$}}

\put(15,90){\makebox(0,0)[cc]{}}

\linethickness{0.3mm}
\put(20,70){\circle*{2.5}}

\linethickness{0.3mm}
\put(40,70){\circle*{2.5}}

\linethickness{0.3mm}
\put(30,70){\circle*{2.5}}

\linethickness{0.3mm}
\put(60,70){\circle*{2.5}}

\linethickness{0.3mm}
\put(50,70){\circle*{2.5}}

\linethickness{0.3mm}
\put(20,60){\circle*{2.5}}

\linethickness{0.3mm}
\put(40,60){\circle*{2.5}}

\linethickness{0.3mm}
\put(30,60){\circle*{2.5}}

\linethickness{0.3mm}
\put(50,60){\circle*{2.5}}

\linethickness{0.3mm}
\put(20,50){\circle*{2.5}}

\linethickness{0.3mm}
\put(40,50){\circle*{2.5}}

\linethickness{0.3mm}
\put(30,50){\circle*{2.5}}

\linethickness{0.3mm}
\put(20,40){\circle*{2.5}}

\linethickness{0.3mm}
\put(30,40){\circle*{2.5}}

\linethickness{0.3mm}
\put(20,30){\circle*{2.5}}

\put(80,5){\makebox(0,0)[cc]{}}

\put(80.62,6.25){\makebox(0,0)[cc]{$t+1$}}

\put(2,80){\makebox(0,0)[cc]{$t+1$}}

\linethickness{0.3mm}
\put(80,8.75){\line(0,1){2.5}}
\linethickness{0.3mm}
\put(8.75,80){\line(1,0){2.5}}
\end{picture}


==> Pstricks/nonregulartriang <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Wed Jul 06 06:24:06 PDT 2011
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-1.25" x-max="61.25" y-min="-1.25" y-max="48.75" auto-bounding="true">
%<ellipse p3= "(1.25,-1.25)"
%	 p2= "(1.25,1.25)"
%	 p1= "(-1.25,1.25)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 fill-style= "solid"
%	 />
%<ellipse p3= "(31.25,46.25)"
%	 p2= "(31.25,48.75)"
%	 p1= "(28.75,48.75)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 fill-style= "solid"
%	 />
%<ellipse p3= "(31.25,26.25)"
%	 p2= "(31.25,28.75)"
%	 p1= "(28.75,28.75)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 fill-style= "solid"
%	 />
%<ellipse p3= "(61.25,-1.25)"
%	 p2= "(61.25,1.25)"
%	 p1= "(58.75,1.25)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 fill-style= "solid"
%	 />
%<ellipse p3= "(41.25,8.75)"
%	 p2= "(41.25,11.25)"
%	 p1= "(38.75,11.25)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 fill-style= "solid"
%	 />
%<ellipse p3= "(21.25,8.75)"
%	 p2= "(21.25,11.25)"
%	 p1= "(18.75,11.25)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 fill-style= "solid"
%	 />
%<multicurve points= "(0,0);(0,0);(60,0);(60,0)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(0,0);(0,0);(30,47.5);(30,47.5)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(30,47.5);(30,47.5);(60,0);(60,0)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(30,27.5);(30,27.5);(40,10);(40,10)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(40,10);(40,10);(20,10);(20,10)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(20,10);(20,10);(30,27.5);(30,27.5)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(0,0);(0,0);(20,10);(20,10)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(0,0);(0,0);(40,10);(40,10)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(60,0);(60,0);(40,10);(40,10)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(60,0);(60,0);(30,27.5);(30,27.5)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(30,47.5);(30,47.5);(30,27.5);(30,27.5)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(30,47.5);(30,47.5);(20,10);(20,10)"
%	 fill-style= "none"
%	 />
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(61.25,48.75)(0,0)
\linethickness{0.3mm}
\put(0,0){\circle*{2.5}}

\linethickness{0.3mm}
\put(30,47.5){\circle*{2.5}}

\linethickness{0.3mm}
\put(30,27.5){\circle*{2.5}}

\linethickness{0.3mm}
\put(60,0){\circle*{2.5}}

\linethickness{0.3mm}
\put(40,10){\circle*{2.5}}

\linethickness{0.3mm}
\put(20,10){\circle*{2.5}}

\linethickness{0.3mm}
\put(0,0){\line(1,0){60}}
\linethickness{0.3mm}
\multiput(0,0)(0.12,0.19){250}{\line(0,1){0.19}}
\linethickness{0.3mm}
\multiput(30,47.5)(0.12,-0.19){250}{\line(0,-1){0.19}}
\linethickness{0.3mm}
\multiput(30,27.5)(0.12,-0.21){83}{\line(0,-1){0.21}}
\linethickness{0.3mm}
\put(20,10){\line(1,0){20}}
\linethickness{0.3mm}
\multiput(20,10)(0.12,0.21){83}{\line(0,1){0.21}}
\linethickness{0.3mm}
\multiput(0,0)(0.24,0.12){83}{\line(1,0){0.24}}
\linethickness{0.3mm}
\multiput(0,0)(0.48,0.12){83}{\line(1,0){0.48}}
\linethickness{0.3mm}
\multiput(40,10)(0.24,-0.12){83}{\line(1,0){0.24}}
\linethickness{0.3mm}
\multiput(30,27.5)(0.13,-0.12){229}{\line(1,0){0.13}}
\linethickness{0.3mm}
\put(30,27.5){\line(0,1){20}}
\linethickness{0.3mm}
\multiput(20,10)(0.12,0.45){83}{\line(0,1){0.45}}
\end{picture}


==> Pstricks/polyhedraintro <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Wed Jul 06 05:48:29 PDT 2011
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-1.25" x-max="149.38" y-min="-1.25" y-max="52.5" auto-bounding="true">
%<multicurve points= "(0,35);(0,35);(0,5);(0,5)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(0,5);(0,5);(30,5);(30,5)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(30,5);(30,5);(30,35);(30,35)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(30,35);(30,35);(0,35);(0,35)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-style= "dashed"
%	 stroke-dasharray= "1;1"
%	 points= "(15,45);(15,45);(15,15);(15,15)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-style= "dashed"
%	 stroke-dasharray= "1;1"
%	 points= "(15,15);(15,15);(45,15);(45,15)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(45,15);(45,15);(45,45);(45,45)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(45,45);(45,45);(15,45);(15,45)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(30,5);(30,5);(45,15);(45,15)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(0,35);(0,35);(15,45);(15,45)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(30,35);(30,35);(45,45);(45,45)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.25"
%	 stroke-style= "dashed"
%	 stroke-dasharray= "1;1"
%	 points= "(0,5);(0,5);(15,15);(15,15)"
%	 fill-style= "none"
%	 />
%<ellipse p3= "(31.25,33.75)"
%	 p2= "(31.25,36.25)"
%	 p1= "(28.75,36.25)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 fill-style= "solid"
%	 />
%<ellipse p3= "(1.25,33.75)"
%	 p2= "(1.25,36.25)"
%	 p1= "(-1.25,36.25)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 fill-style= "solid"
%	 />
%<ellipse p3= "(1.25,3.75)"
%	 p2= "(1.25,6.25)"
%	 p1= "(-1.25,6.25)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 fill-style= "solid"
%	 />
%<ellipse p3= "(16.25,13.75)"
%	 p2= "(16.25,16.25)"
%	 p1= "(13.75,16.25)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 fill-style= "solid"
%	 />
%<ellipse p3= "(16.25,43.75)"
%	 p2= "(16.25,46.25)"
%	 p1= "(13.75,46.25)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 fill-style= "solid"
%	 />
%<ellipse p3= "(46.25,43.75)"
%	 p2= "(46.25,46.25)"
%	 p1= "(43.75,46.25)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 fill-style= "solid"
%	 />
%<ellipse p3= "(46.25,13.75)"
%	 p2= "(46.25,16.25)"
%	 p1= "(43.75,16.25)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 fill-style= "solid"
%	 />
%<ellipse p3= "(31.25,3.75)"
%	 p2= "(31.25,6.25)"
%	 p1= "(28.75,6.25)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 fill-style= "solid"
%	 />
%<multicurve points= "(75,30);(75,30);(75,0);(75,0)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(75,0);(75,0);(105,0);(105,0)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(105,0);(105,0);(105,30);(105,30)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(105,30);(105,30);(75,30);(75,30)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(105,0);(105,0);(149.38,20);(149.38,20)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(75,30);(75,30);(98.12,52.5);(98.12,52.5)"
%	 fill-style= "none"
%	 />
%<multicurve points= "(105,30);(105,30);(143.75,52.5);(143.75,52.5)"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.25"
%	 stroke-style= "dashed"
%	 stroke-dasharray= "1;1"
%	 points= "(75,0);(75,0);(98.75,15);(98.75,15)"
%	 fill-style= "none"
%	 />
%<ellipse p3= "(106.25,28.75)"
%	 p2= "(106.25,31.25)"
%	 p1= "(103.75,31.25)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 fill-style= "solid"
%	 />
%<ellipse p3= "(76.25,28.75)"
%	 p2= "(76.25,31.25)"
%	 p1= "(73.75,31.25)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 fill-style= "solid"
%	 />
%<ellipse p3= "(76.25,-1.25)"
%	 p2= "(76.25,1.25)"
%	 p1= "(73.75,1.25)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 fill-style= "solid"
%	 />
%<ellipse p3= "(106.25,-1.25)"
%	 p2= "(106.25,1.25)"
%	 p1= "(103.75,1.25)"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 fill-style= "solid"
%	 />
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(149.38,52.5)(0,0)
\linethickness{0.3mm}
\put(0,5){\line(0,1){30}}
\linethickness{0.3mm}
\put(0,5){\line(1,0){30}}
\linethickness{0.3mm}
\put(30,5){\line(0,1){30}}
\linethickness{0.3mm}
\put(0,35){\line(1,0){30}}
\linethickness{0.3mm}
\multiput(15,15)(0,1.94){16}{\line(0,1){0.97}}
\linethickness{0.3mm}
\multiput(15,15)(1.94,0){16}{\line(1,0){0.97}}
\linethickness{0.3mm}
\put(45,15){\line(0,1){30}}
\linethickness{0.3mm}
\put(15,45){\line(1,0){30}}
\linethickness{0.3mm}
\multiput(30,5)(0.18,0.12){83}{\line(1,0){0.18}}
\linethickness{0.3mm}
\multiput(0,35)(0.18,0.12){83}{\line(1,0){0.18}}
\linethickness{0.3mm}
\multiput(30,35)(0.18,0.12){83}{\line(1,0){0.18}}
\linethickness{0.25mm}
\multiput(0,5)(1.58,1.05){10}{\multiput(0,0)(0.2,0.13){4}{\line(1,0){0.2}}}
\linethickness{0.3mm}
\put(30,35){\circle*{2.5}}

\linethickness{0.3mm}
\put(0,35){\circle*{2.5}}

\linethickness{0.3mm}
\put(0,5){\circle*{2.5}}

\linethickness{0.3mm}
\put(15,15){\circle*{2.5}}

\linethickness{0.3mm}
\put(15,45){\circle*{2.5}}

\linethickness{0.3mm}
\put(45,45){\circle*{2.5}}

\linethickness{0.3mm}
\put(45,15){\circle*{2.5}}

\linethickness{0.3mm}
\put(30,5){\circle*{2.5}}

\linethickness{0.3mm}
\put(75,0){\line(0,1){30}}
\linethickness{0.3mm}
\put(75,0){\line(1,0){30}}
\linethickness{0.3mm}
\put(105,0){\line(0,1){30}}
\linethickness{0.3mm}
\put(75,30){\line(1,0){30}}
\linethickness{0.3mm}
\multiput(105,0)(0.27,0.12){167}{\line(1,0){0.27}}
\linethickness{0.3mm}
\multiput(75,30)(0.12,0.12){188}{\line(1,0){0.12}}
\linethickness{0.3mm}
\multiput(105,30)(0.21,0.12){188}{\line(1,0){0.21}}
\linethickness{0.25mm}
\multiput(75,0)(1.64,1.03){15}{\multiput(0,0)(0.2,0.13){4}{\line(1,0){0.2}}}
\linethickness{0.3mm}
\put(105,30){\circle*{2.5}}

\linethickness{0.3mm}
\put(75,30){\circle*{2.5}}

\linethickness{0.3mm}
\put(75,0){\circle*{2.5}}

\linethickness{0.3mm}
\put(105,0){\circle*{2.5}}

\end{picture}


==> Pstricks/titlepic <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Fri Jul 15 12:24:05 PDT 2011
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="5" x-max="170" y-min="-0.01" y-max="50" auto-bounding="true">
%<ellipse p3= "(46.25,33.75)"
%	 p2= "(46.25,36.25)"
%	 p1= "(43.75,36.25)"
%	 closure= "open"
%	 fill-style= "solid"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve right-arrow= "head"
%	 stroke-width= "0.05"
%	 fill-style= "none"
%	 points= "(5,25);(5,25);(50,25);(50,25)"
%	 />
%<multicurve stroke-width= "0.05"
%	 left-arrow= "head"
%	 fill-style= "none"
%	 stroke-color= "#cccccc"
%	 points= "(25,50);(25,50);(25,0);(25,0)"
%	 />
%<ellipse p3= "(16.25,33.75)"
%	 p2= "(16.25,36.25)"
%	 p1= "(13.75,36.25)"
%	 closure= "open"
%	 fill-style= "solid"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25,25);(25,25);(45,35);(45,35)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,35);(15,35);(25,25);(25,25)"
%	 />
%<multicurve stroke-style= "dashed"
%	 stroke-dasharray= "1;1"
%	 fill-style= "none"
%	 points= "(15,35);(15,35);(35,45);(35,45)"
%	 />
%<multicurve stroke-style= "dashed"
%	 stroke-dasharray= "1;1"
%	 fill-style= "none"
%	 points= "(45,35);(45,35);(35,45);(35,45)"
%	 />
%<multicurve right-arrow= "head"
%	 stroke-width= "0.05"
%	 fill-style= "none"
%	 points= "(65,25);(65,25);(110,25);(110,25)"
%	 />
%<multicurve stroke-width= "0.05"
%	 left-arrow= "head"
%	 fill-style= "none"
%	 points= "(85,50);(85,50);(85,0);(85,0)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(65,15);(65,15);(85,25);(85,25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(85,25);(85,25);(95,15);(95,15)"
%	 />
%<multicurve stroke-style= "dashed"
%	 stroke-dasharray= "1;1"
%	 fill-style= "none"
%	 points= "(75,5);(75,5);(95,15);(95,15)"
%	 />
%<multicurve stroke-style= "dashed"
%	 stroke-dasharray= "1;1"
%	 fill-style= "none"
%	 points= "(75,5);(75,5);(65,15);(65,15)"
%	 />
%<multicurve right-arrow= "head"
%	 stroke-width= "0.05"
%	 fill-style= "none"
%	 points= "(125,25);(125,25);(170,25);(170,25)"
%	 />
%<multicurve stroke-width= "0.05"
%	 left-arrow= "head"
%	 fill-style= "none"
%	 points= "(145,50);(145,50);(145,-0.01);(145,-0.01)"
%	 />
%<multicurve stroke-style= "dashed"
%	 stroke-dasharray= "1;1"
%	 fill-style= "none"
%	 points= "(145,25);(145,25);(165,35);(165,35)"
%	 />
%<multicurve stroke-style= "dashed"
%	 stroke-dasharray= "1;1"
%	 fill-style= "none"
%	 points= "(135,35);(135,35);(145,25);(145,25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(135,35);(135,35);(155,45);(155,45)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(165,35);(165,35);(155,45);(155,45)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(30,35.62)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Q$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(78.75,15)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$-\Q$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(5,35)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(11.25,35.62)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\v$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(49.38,35)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\w$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(149.38,35)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$-\Q+\v+\w$
%</text>
%</jpic>
%%End JPIC-XML
%LaTeX-picture environment using emulated lines and arcs
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\unitlength \JPicScale mm
\begin{picture}(170,50)(0,0)
\linethickness{0.3mm}
\put(45,35){\circle*{2.5}}

\linethickness{0.05mm}
\put(5,25){\line(1,0){45}}
\put(50,25){\vector(1,0){0.12}}
\linethickness{0.05mm}
\put(25,0){\line(0,1){50}}
\put(25,50){\vector(0,1){0.12}}
\linethickness{0.3mm}
\put(15,35){\circle*{2.5}}

\linethickness{0.3mm}
\multiput(25,25)(0.24,0.12){83}{\line(1,0){0.24}}
\linethickness{0.3mm}
\multiput(15,35)(0.12,-0.12){83}{\line(1,0){0.12}}
\linethickness{0.3mm}
\multiput(15,35)(1.74,0.87){12}{\multiput(0,0)(0.22,0.11){4}{\line(1,0){0.22}}}
\linethickness{0.3mm}
\multiput(35,45)(1.33,-1.33){8}{\multiput(0,0)(0.11,-0.11){6}{\line(1,0){0.11}}}
\linethickness{0.05mm}
\put(65,25){\line(1,0){45}}
\put(110,25){\vector(1,0){0.12}}
\linethickness{0.05mm}
\put(85,0){\line(0,1){50}}
\put(85,50){\vector(0,1){0.12}}
\linethickness{0.3mm}
\multiput(65,15)(0.24,0.12){83}{\line(1,0){0.24}}
\linethickness{0.3mm}
\multiput(85,25)(0.12,-0.12){83}{\line(1,0){0.12}}
\linethickness{0.3mm}
\multiput(75,5)(1.74,0.87){12}{\multiput(0,0)(0.22,0.11){4}{\line(1,0){0.22}}}
\linethickness{0.3mm}
\multiput(65,15)(1.33,-1.33){8}{\multiput(0,0)(0.11,-0.11){6}{\line(1,0){0.11}}}
\linethickness{0.05mm}
\put(125,25){\line(1,0){45}}
\put(170,25){\vector(1,0){0.12}}
\linethickness{0.05mm}
\put(145,-0.01){\line(0,1){50}}
\put(145,50){\vector(0,1){0.12}}
\linethickness{0.3mm}
\multiput(145,25)(1.74,0.87){12}{\multiput(0,0)(0.22,0.11){4}{\line(1,0){0.22}}}
\linethickness{0.3mm}
\multiput(135,35)(1.33,-1.33){8}{\multiput(0,0)(0.11,-0.11){6}{\line(1,0){0.11}}}
\linethickness{0.3mm}
\multiput(135,35)(0.24,0.12){83}{\line(1,0){0.24}}
\linethickness{0.3mm}
\multiput(155,45)(0.12,-0.12){83}{\line(1,0){0.12}}
\put(30,35.62){\makebox(0,0)[cc]{$\Q$}}

\put(78.75,15){\makebox(0,0)[cc]{$-\Q$}}

\put(5,35){\makebox(0,0)[cc]{}}

\put(11.25,35.62){\makebox(0,0)[cc]{$\v$}}

\put(49.38,35){\makebox(0,0)[cc]{$\w$}}

\put(149.38,35){\makebox(0,0)[cc]{$-\Q+\v+\w$}}

\end{picture}

